Contextual Semibandits via Supervised Learning Oracles

We study an online decision making problem where on each round a learner chooses a list of items based on some side information, receives a scalar feedback value for each individual item, and a reward that is linearly related to this feedback. These problems, known as contextual semibandits, arise in crowdsourcing, recommendation, and many other domains. This paper reduces contextual semibandits to supervised learning, allowing us to leverage powerful supervised learning methods in this partial-feedback setting. Our first reduction applies when the mapping from feedback to reward is known and leads to a computationally efficient algorithm with near-optimal regret. We show that this algorithm outperforms state-of-the-art approaches on real-world learning-to-rank datasets, demonstrating the advantage of oracle-based algorithms. Our second reduction applies to the previously unstudied setting when the linear mapping from feedback to reward is unknown. Our regret guarantees are superior to prior techniques that ignore the feedback.

==> table.tex <==
\section{Table comparing results}

\begin{table}
\begin{tabular}{|c|c|c|c|}
\hline
Algorithm & Regret & Oracle Calls & Weights Known?\\
\hline\hline
\semimonster & $\sqrt{KLT\logN}$ & $T^{3/2}\sqrt{K/(L\logN)}$ & Yes\\
\hline
$\epsilon$-Greedy & $(TL)^{2/3}(K\logN)^{1/3}$ & $1$ & Yes\\
\hline
\citet{kale2010non} & $\sqrt{KLT\logN}$ & Not oracle-based & Yes\\
\hline
\eels & $(TL)^{2/3}(K\logN)^{1/3}$ & $1$ & No\\
\hline
\citet{agarwal2014taming} & $\sqrt{K^LT\logN}$ & $\sqrt{K^LT/\logN}$ & No\\
\hline
\citet{swaminathan2016off} & $LT^{2/3}(K\logN)^{1/3}$ & $1$ & No\\
\hline
\end{tabular}
\caption{Comparison of regret and running time, measured by oracle
  calls, of algorithms that can be applied naively to our setting.
  Bounds in the table are specialized to $\ws = \mathbf{1}$ or $B =
  \Theta(\sqrt{L})$ and $\pmin = \Omega(L)$.}
\end{table}

\section{Analysis of $\epsilon$-Greedy with Known Weights}
We analyze the $\epsilon$-greedy algorithm in the known weights setting when uniform exploration is valid (i.e. $\pmin = L$). Pseudocode for the algorithm is in Algorithm~\ref{alg:eps_greedy}.

\begin{algorithm}[t]
\caption{$\epsilon$-Greedy for Contextual Semibandits with Known Weights}
\label{alg:eps_greedy}
\begin{algorithmic}[t]
\REQUIRE Allowed failure probability $\delta \in (0,1)$.
\STATE Set $n = T^{2/3}(K\log(2N/\delta)/L)^{1/3}$.
\STATE For $t=1,\ldots, n$, observe $x_t$, play $A_t \sim U$, observe $y_t(A_t)$ and $r_t(A_t)$.
\STATE Optimize policy $\hat{\pi} \gets \argmax_{\pi \in \Pi} \eta_n(\pi,\ws)$ using importance weighted features.
\STATE For every remaining round: observe $x_t$, play $A_t = \hat{\pi}(x_t)$.
\end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:eps_greedy}
For any $\delta \in (0,1)$, when $T \ge \frac{\log (N/\delta)}{L\sqrt{K}}$, with probability at least $1-\delta$, the regret of Algorithm~\ref{alg:eps_greedy} is at most $\otil(\|\ws\|T(K\log(N/\delta))^{1/3}L^{1/6})$.
\end{theorem}
\begin{proof}
The proof relies on the uniform deviation bound, which is essentially the same as Lemma~\ref{lem:eels_reward_deviation} that we use for the analysis of \eels.
We first prove, that for any $\delta \in (0,1)$, with probability at least $1-\delta$, for all policies $\pi$, we have,
\begin{align}
|\eta_n(\pi,\ws) - \Rcal(\pi)| \le 2\|\ws\|\left(\sqrt{\frac{K\log(2N/\delta)}{n}} + \sqrt{\frac{K}{L}}\frac{\log(2N/\delta)}{n}\right). \label{eq:eps_greedy_deviation}
\end{align}
This deviation bound is a consequence of Bernstein's inequality.
Clearly the quantity on the left hand side is centered, since $\Rcal(\pi) = \EE_{x,y}y_\pi^T\ws$.
The range of each term is,
\begin{align*}
\hat{y}_i(\pi)^T \ws - \EE_{x,y} y_\pi^T \ws \le \|\ws\| \|\hat{y}_i(\pi) - \EE_{x,y} y_\pi \|
\le \|\ws\|\sqrt{K^2/L}
\end{align*}
This last inequality is based on the fact that with uniform exploration, the coordinates of $\hat{y}_i(\pi)$ are bounded in $[0,K/L]$ while the coordinates of $y_\pi$ are in $[0,1]$ and these are $L$-dimensional vectors.
The variance is bounded by the second moment, which can be further bounded as,
\begin{align*}
\EE_{x,y,A}( \hat{y}_\pi^T\ws)^2 \le \|\ws\|^2 \EE_{x,y,A}\sum_{l=1}^L\hat{y}(\pi(x_l))^2 \le \|\ws\|^2\EE_{x,y,A} \sum_{l=1}^L \frac{K^2}{L^2}\mathbf{1}(\pi(x)_l \in A)
 = \|\ws\|^2K.
\end{align*}
Since $\EE_{x,y,A}\mathbf{1}(\pi(x)_l \in A) = L/K$ since we are using uniform exploration.
Plugging in these bounds into Bernstein's inequality gives the deviation bound.

Now we can prove the theorem.
Eq.~\eqref{eq:eps_greedy_deviation} ensures that after collecting $n$ samples, the expected reward of the empirical reward maximizer $\hat{\pi}$ is close to $\max_\pi \Rcal(\pi)$, the best achievable reward.
The difference between these two is at most twice the right hand side of the deviation bound.
If we perform uniform exploration for $n$ rounds, we are ensured that the regret is at most,
\begin{align*}
\textrm{Regret} & \le  n \|\ws\|\sqrt{L} + (T-n)4\|\ws\|\left(\sqrt{\frac{K\log(2N/\delta)}{n}} + \sqrt{\frac{K}{L}}\frac{\log(2N/\delta)}{n}\right)\\
& \le n \|\ws\|\sqrt{L} + 4T\|\ws\|\left(\sqrt{\frac{K\log(2N/\delta)}{n}} + \sqrt{\frac{K}{L}}\frac{\log(2N/\delta)}{n}\right)
\end{align*}
Set $n = T^{2/3}(K\log(2N/\delta)/L)^{1/3}$, the bound is,
\begin{align*}
5 \|\ws\| T^{2/3}(K\log(2N/\delta))^{1/3}L^{1/6} + 4\|\ws\|T^{1/3}K^{1/6}\log(2N/\delta)^{2/3}L^{-1/6}.
\end{align*}
Under the assumption on $T$, the second term is lower order, which proves the result.
\end{proof}

